SLM-Bench: A Comprehensive Benchmark of Small Language Models on Environmental Impacts--Extended Version

Small Language Models (SLMs) offer computational efficiency and accessibility, yet a systematic evaluation of their performance and environmental impact remains lacking. We introduce SLM-Bench, the first benchmark specifically designed to assess SLMs across multiple dimensions, including accuracy, computational efficiency, and sustainability metrics. SLM-Bench evaluates 15 SLMs on 9 NLP tasks using 23 datasets spanning 14 domains. The evaluation is conducted on 4 hardware configurations, providing a rigorous comparison of their effectiveness. Unlike prior benchmarks, SLM-Bench quantifies 11 metrics across correctness, computation, and consumption, enabling a holistic assessment of efficiency trade-offs. Our evaluation considers controlled hardware conditions, ensuring fair comparisons across models. We develop an open-source benchmarking pipeline with standardized evaluation protocols to facilitate reproducibility and further research. Our findings highlight the diverse trade-offs among SLMs, where some models excel in accuracy while others achieve superior energy efficiency. SLM-Bench sets a new standard for SLM evaluation, bridging the gap between resource efficiency and real-world applicability.

==> tables/app-result-details-L4.tex <==
\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B}      & 0.389                & 0.272      & 0.232        & 0.136              & 505,700              & 0.718    & 0.696    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Phi-1.5}           & 0.293                & 0.205      & 0.174        & 0.102              & 2,136,973             & 0.778    & 0.755    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Open-Llama-3B}     & 0.74                 & 0.518      & 0.441        & 0.259              & 2,220,000             & 0.749    & 0.725    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Llama-2-7B}        & 0.324                & 0.227      & 0.193        & 0.113              & 2,268,000             & 0.794    & 0.774    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Mistral-7B}        & 0.927                & 0.649      & 0.552        & 0.324              & 6,489,000             & 0.764    & 0.745    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Zephyr-7B}         & 0.531                & 0.372      & 0.316        & 0.186              & 3,717,000             & 0.823    & 0.804    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{TinyLlama-1.1B}    & 0.694                & 0.486      & 0.413        & 0.243              & 763,400              & 0.673    & 0.657    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{StableLM-3B}       & 0.342                & 0.239      & 0.204        & 0.12               & 1,026,000             & 0.694    & 0.676    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{ShearedLlama-2.7B} & 0.869                & 0.608      & 0.517        & 0.304              & 2,346,300             & 0.745    & 0.725    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Dolly-v2-3B}       & 0.296                & 0.207      & 0.176        & 0.104              & 888,000              & 0.779    & 0.755    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Pythia-2.8B}       & 0.357                & 0.25       & 0.213        & 0.125              & 999,600              & 0.742    & 0.725    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Gemma-2B}          & 0.861                & 0.603      & 0.513        & 0.301              & 1,722,000             & 0.762    & 0.735    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Llama-3.2-1B}      & 1.023                & 0.716      & 0.388        & 0.28               & 8,500,000             & 0.935    & 0.892    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Phi-3}             & 0.959                & 0.671      & 0.371        & 0.258              & 7,200,000             & 0.856    & 0.784    & N/A  & N/A   & N/A    & N/A        \\
    \texttt{Gemma-3}           & 1.037                & 0.726      & 0.393        & 0.271              & 6,800,000             & 0.923    & 0.881    & N/A  & N/A   & N/A    & N/A        \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{BoolQ}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}

\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.295 & 0.206 & 0.176 & 0.103 & 383,500  & 0.624 & 0.608 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-1.5} & 0.878 & 0.615 & 0.523 & 0.307 & 2,136,973 & 0.603 & 0.588 & N/A & N/A & N/A & N/A \\
    \texttt{Open-Llama-3B} & 0.932 & 0.652 & 0.555 & 0.326 & 2,796,000 & 0.678 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-2-7B} & 0.46  & 0.322 & 0.274 & 0.161 & 3,220,000 & 0.686 & 0.666 & N/A & N/A & N/A & N/A \\
    \texttt{Mistral-7B} & 0.591 & 0.414 & 0.352 & 0.207 & 4,137,000 & 0.628 & 0.608 & N/A & N/A & N/A & N/A \\
    \texttt{Zephyr-7B} & 0.593 & 0.415 & 0.353 & 0.207 & 4,151,000 & 0.734 & 0.706 & N/A & N/A & N/A & N/A \\
    \texttt{TinyLlama-1.1B} & 0.85  & 0.595 & 0.506 & 0.297 & 935,000  & 0.679 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{StableLM-3B} & 0.812 & 0.568 & 0.483 & 0.284 & 2,436,000 & 0.672 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{ShearedLlama-2.7B} & 0.734 & 0.514 & 0.437 & 0.257 & 1,981,800 & 0.674 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{Dolly-v2-3B} & 0.273 & 0.191 & 0.163 & 0.095 & 819,000  & 0.709 & 0.686 & N/A & N/A & N/A & N/A \\
    \texttt{Pythia-2.8B} & 0.915 & 0.64  & 0.545 & 0.32  & 2,562,000 & 0.678 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-2B} & 0.448 & 0.314 & 0.267 & 0.157 & 896,000  & 0.569 & 0.549 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-3.2-1B} & 0.818 & 0.573 & 0.302 & 0.21  & 8,500,000 & 0.933 & 0.884 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-3} & 0.758 & 0.531 & 0.289 & 0.198 & 7,200,000 & 0.874 & 0.822 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-3} & 0.789 & 0.552 & 0.306 & 0.212 & 6,800,000 & 0.923 & 0.87  & N/A & N/A & N/A & N/A \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{ARC-Challenge}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}

\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.905 & 0.634 & 0.539 & 0.317 & 1,176,500 & 0.809 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-1.5} & 0.648 & 0.454 & 0.386 & 0.227 & 2,136,973 & 0.738 & 0.715 & N/A & N/A & N/A & N/A \\
    \texttt{Open-Llama-3B} & 0.723 & 0.506 & 0.43  & 0.253 & 2,169,000 & 0.767 & 0.745 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-2-7B} & 0.208 & 0.146 & 0.124 & 0.073 & 1,456,000 & 0.756 & 0.735 & N/A & N/A & N/A & N/A \\
    \texttt{Mistral-7B} & 0.329 & 0.23  & 0.196 & 0.115 & 2,303,000 & 0.802 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{Zephyr-7B} & 0.531 & 0.372 & 0.316 & 0.186 & 3,717,000 & 0.769 & 0.745 & N/A & N/A & N/A & N/A \\
    \texttt{TinyLlama-1.1B} & 0.534 & 0.374 & 0.318 & 0.187 & 587,400   & 0.799 & 0.774 & N/A & N/A & N/A & N/A \\
    \texttt{StableLM-3B} & 0.565 & 0.395 & 0.336 & 0.198 & 1,695,000 & 0.809 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{ShearedLlama-2.7B} & 0.893 & 0.625 & 0.532 & 0.312 & 2,411,100 & 0.771 & 0.745 & N/A & N/A & N/A & N/A \\
    \texttt{Dolly-v2-3B} & 0.846 & 0.592 & 0.504 & 0.296 & 2,538,000 & 0.804 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{Pythia-2.8B} & 0.993 & 0.695 & 0.591 & 0.347 & 2,780,400 & 0.739 & 0.706 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-2B} & 0.275 & 0.192 & 0.164 & 0.096 & 550,000   & 0.739 & 0.715 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-3.2-1B} & 1.163 & 0.814 & 0.43  & 0.3   & 8,500,000 & 0.831 & 0.785 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-3} & 1.132 & 0.792 & 0.422 & 0.301 & 7,200,000 & 0.859 & 0.776 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-3} & 1.226 & 0.858 & 0.456 & 0.331 & 6,800,000 & 0.809 & 0.741 & N/A & N/A & N/A & N/A \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{PIQA}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}

\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.828 & 0.58  & 0.493 & 0.29  & 1,076,400 & 0.798 & 0.774 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-1.5} & 0.343 & 0.24  & 0.204 & 0.12  & 2,136,972 & 0.765 & 0.745 & N/A & N/A & N/A & N/A \\
    \texttt{Open-Llama-3B} & 0.261 & 0.183 & 0.155 & 0.091 & 783,000   & 0.762 & 0.745 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-2-7B} & 0.551 & 0.386 & 0.328 & 0.193 & 3,857,000 & 0.804 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{Mistral-7B} & 0.27  & 0.189 & 0.161 & 0.094 & 1,890,000 & 0.849 & 0.823 & N/A & N/A & N/A & N/A \\
    \texttt{Zephyr-7B} & 0.621 & 0.435 & 0.37  & 0.217 & 4,347,000 & 0.859 & 0.833 & N/A & N/A & N/A & N/A \\
    \texttt{TinyLlama-1.1B} & 0.28  & 0.196 & 0.167 & 0.098 & 308,000   & 0.757 & 0.725 & N/A & N/A & N/A & N/A \\
    \texttt{StableLM-3B} & 0.325 & 0.227 & 0.194 & 0.114 & 975,000   & 0.808 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{ShearedLlama-2.7B} & 0.997 & 0.698 & 0.594 & 0.349 & 2,691,900 & 0.757 & 0.735 & N/A & N/A & N/A & N/A \\
    \texttt{Dolly-v2-3B} & 0.893 & 0.625 & 0.532 & 0.312 & 2,679,000 & 0.794 & 0.774 & N/A & N/A & N/A & N/A \\
    \texttt{Pythia-2.8B} & 0.824 & 0.577 & 0.491 & 0.288 & 2,307,200 & 0.774 & 0.755 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-2B} & 0.648 & 0.454 & 0.386 & 0.227 & 1,296,000 & 0.746 & 0.725 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-3.2-1B} & 1.262 & 0.883 & 0.483 & 0.345 & 8,500,000 & 0.831 & 0.772 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-3} & 1.234 & 0.864 & 0.474 & 0.331 & 7,200,000 & 0.851 & 0.774 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-3} & 1.386 & 0.97  & 0.515 & 0.367 & 6,800,000 & 0.822 & 0.765 & N/A & N/A & N/A & N/A \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{WinoGrande}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}

\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.237 & 0.166 & 0.141 & 0.083 & 308,100   & 0.446 & 0.431 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-1.5} & 0.821 & 0.575 & 0.489 & 0.287 & 2,136,972 & 0.547 & 0.529 & N/A & N/A & N/A & N/A \\
    \texttt{Open-Llama-3B} & 0.811 & 0.568 & 0.483 & 0.284 & 2,433,000 & 0.514 & 0.598 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-2-7B} & 0.378 & 0.265 & 0.225 & 0.132 & 2,646,000 & 0.563 & 0.539 & N/A & N/A & N/A & N/A \\
    \texttt{Mistral-7B} & 0.358 & 0.251 & 0.213 & 0.125 & 2,506,000 & 0.566 & 0.549 & N/A & N/A & N/A & N/A \\
    \texttt{Zephyr-7B} & 0.315 & 0.22  & 0.188 & 0.11  & 2,205,000 & 0.576 & 0.559 & N/A & N/A & N/A & N/A \\
    \texttt{TinyLlama-1.1B} & 0.564 & 0.395 & 0.336 & 0.197 & 620,400   & 0.546 & 0.529 & N/A & N/A & N/A & N/A \\
    \texttt{StableLM-3B} & 0.204 & 0.143 & 0.121 & 0.071 & 612,000   & 0.499 & 0.489 & N/A & N/A & N/A & N/A \\
    \texttt{ShearedLlama-2.7B} & 0.476 & 0.333 & 0.283 & 0.167 & 1,285,200 & 0.479 & 0.461 & N/A & N/A & N/A & N/A \\
    \texttt{Dolly-v2-3B} & 0.236 & 0.165 & 0.141 & 0.083 & 708,000   & 0.517 & 0.553 & N/A & N/A & N/A & N/A \\
    \texttt{Pythia-2.8B} & 0.836 & 0.585 & 0.498 & 0.292 & 2,340,800 & 0.455 & 0.441 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-2B} & 0.407 & 0.285 & 0.242 & 0.142 & 814,000   & 0.447 & 0.431 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-3.2-1B} & 1.149 & 0.804 & 0.444 & 0.317 & 8,500,000 & 0.832 & 0.784 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-3} & 1.122 & 0.785 & 0.414 & 0.287 & 7,200,000 & 0.775 & 0.729 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-3} & 1.171 & 0.82  & 0.438 & 0.318 & 6,800,000 & 0.787 & 0.745 & N/A & N/A & N/A & N/A \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{GSM8k}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}


\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.347 & 0.243 & 0.207 & 0.121 & 451,100   & 0.663 & 0.647 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-1.5} & 0.405 & 0.284 & 0.241 & 0.142 & 2,136,972 & 0.672 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{Open-Llama-3B} & 0.523 & 0.366 & 0.311 & 0.183 & 1,569,000 & 0.596 & 0.578 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-2-7B} & 0.875 & 0.612 & 0.521 & 0.306 & 6,125,000 & 0.634 & 0.617 & N/A & N/A & N/A & N/A \\
    \texttt{Mistral-7B} & 0.718 & 0.503 & 0.427 & 0.251 & 5,026,000 & 0.741 & 0.715 & N/A & N/A & N/A & N/A \\
    \texttt{Zephyr-7B} & 0.706 & 0.494 & 0.42  & 0.247 & 4,942,000 & 0.662 & 0.637 & N/A & N/A & N/A & N/A \\
    \texttt{TinyLlama-1.1B} & 0.977 & 0.684 & 0.582 & 0.342 & 1,074,700 & 0.664 & 0.637 & N/A & N/A & N/A & N/A \\
    \texttt{StableLM-3B} & 0.896 & 0.627 & 0.533 & 0.313 & 2,688,000 & 0.727 & 0.696 & N/A & N/A & N/A & N/A \\
    \texttt{ShearedLlama-2.7B} & 0.555 & 0.388 & 0.33  & 0.194 & 1,498,500 & 0.637 & 0.617 & N/A & N/A & N/A & N/A \\
    \texttt{Dolly-v2-3B} & 0.885 & 0.619 & 0.527 & 0.31  & 2,655,000 & 0.703 & 0.686 & N/A & N/A & N/A & N/A \\
    \texttt{Pythia-2.8B} & 0.769 & 0.538 & 0.458 & 0.269 & 2,153,200 & 0.572 & 0.559 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-2B} & 0.563 & 0.394 & 0.335 & 0.197 & 1,126,000 & 0.625 & 0.608 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-3.2-1B} & 1.147 & 0.803 & 0.442 & 0.309 & 8,500,000 & 0.871 & 0.818 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-3} & 1.102 & 0.771 & 0.405 & 0.28  & 7,200,000 & 0.831 & 0.767 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-3} & 1.126 & 0.788 & 0.43  & 0.299 & 6,800,000 & 0.907 & 0.87  & N/A & N/A & N/A & N/A \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{RACE-Middle}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}


\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.773 & 0.541 & 0.46  & 0.27  & 1,004,900 & 0.683 & 0.666 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-1.5} & 0.227 & 0.159 & 0.135 & 0.079 & 2,136,972 & 0.744 & 0.676 & N/A & N/A & N/A & N/A \\
    \texttt{Open-Llama-3B} & 0.742 & 0.519 & 0.442 & 0.26  & 2,226,000 & 0.678 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-2-7B} & 0.504 & 0.353 & 0.3   & 0.176 & 3,528,000 & 0.762 & 0.745 & N/A & N/A & N/A & N/A \\
    \texttt{Mistral-7B} & 0.802 & 0.561 & 0.478 & 0.281 & 5,614,000 & 0.747 & 0.715 & N/A & N/A & N/A & N/A \\
    \texttt{Zephyr-7B} & 0.574 & 0.402 & 0.342 & 0.201 & 4,018,000 & 0.796 & 0.774 & N/A & N/A & N/A & N/A \\
    \texttt{TinyLlama-1.1B} & 0.862 & 0.603 & 0.513 & 0.302 & 948,200   & 0.684 & 0.666 & N/A & N/A & N/A & N/A \\
    \texttt{StableLM-3B} & 0.755 & 0.528 & 0.45  & 0.264 & 2,265,000 & 0.729 & 0.706 & N/A & N/A & N/A & N/A \\
    \texttt{ShearedLlama-2.7B} & 0.791 & 0.554 & 0.471 & 0.277 & 2,135,700 & 0.745 & 0.725 & N/A & N/A & N/A & N/A \\
    \texttt{Dolly-v2-3B} & 0.752 & 0.526 & 0.448 & 0.263 & 2,256,000 & 0.718 & 0.696 & N/A & N/A & N/A & N/A \\
    \texttt{Pythia-2.8B} & 0.623 & 0.436 & 0.371 & 0.218 & 1,744,400 & 0.689 & 0.666 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-2B} & 0.88  & 0.616 & 0.524 & 0.308 & 1,760,000 & 0.674 & 0.657 & N/A & N/A & N/A & N/A \\
    \texttt{Llama-3.2-1B} & 1.254 & 0.878 & 0.476 & 0.334 & 8,500,000 & 0.934 & 0.867 & N/A & N/A & N/A & N/A \\
    \texttt{Phi-3} & 1.14  & 0.798 & 0.424 & 0.302 & 7,200,000 & 0.903 & 0.835 & N/A & N/A & N/A & N/A \\
    \texttt{Gemma-3} & 1.242 & 0.869 & 0.481 & 0.332 & 6,800,000 & 0.888 & 0.807 & N/A & N/A & N/A & N/A \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{CoQA}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}


\begin{table*}[h]
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{2}{blue!7}{white}
    \fontsize{7.5}{7.5}\selectfont
    \setlength{\tabcolsep}{1.8pt}
    \centering
    \begin{tabularx}{\textwidth}{lp{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}p{1.5cm}lp{0.8cm}llll}
    \rowcolor{white}
    \toprule
    \textbf{Model}             & \textbf{Fine-tuning Time} (h) & \textbf{Cost} (USD) & \textbf{Energy} (kWh) & \textbf{CO2 Emissions} (kg) & \textbf{Complexity} (TFLOPS) & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{Perplexity} \\
    \midrule
    \texttt{GPT-Neo-1.3B} & 0.655 & 0.458 & 0.39  & 0.229 & 851,500   & N/A & N/A & 0.667 & 0.792 & 0.726 & 1.312 \\
    \texttt{Phi-1.5} & 0.866 & 0.606 & 0.516 & 0.303 & 2,136,972 & N/A & N/A & 0.638 & 0.756 & 0.693 & 1.356 \\
    \texttt{Open-Llama-3B} & 0.329 & 0.23  & 0.196 & 0.115 & 987,000   & N/A & N/A & 0.686 & 0.816 & 0.748 & 1.284 \\
    \texttt{Llama-2-7B} & 0.286 & 0.2   & 0.17  & 0.1   & 2,002,000 & N/A & N/A & 0.664 & 0.792 & 0.726 & 1.313 \\
    \texttt{Mistral-7B} & 0.761 & 0.533 & 0.453 & 0.266 & 5,327,000 & N/A & N/A & 0.752 & 0.989 & 0.825 & 1.156 \\
    \texttt{Zephyr-7B} & 0.474 & 0.332 & 0.282 & 0.166 & 3,318,000 & N/A & N/A & 0.681 & 0.804 & 0.737 & 1.296 \\
    \texttt{TinyLlama-1.1B} & 0.531 & 0.372 & 0.316 & 0.186 & 584,100   & N/A & N/A & 0.707 & 0.842 & 0.771 & 1.254 \\
    \texttt{StableLM-3B} & 0.362 & 0.253 & 0.216 & 0.127 & 1,086,000 & N/A & N/A & 0.636 & 0.756 & 0.693 & 1.357 \\
    \texttt{ShearedLlama-2.7B} & 0.277 & 0.194 & 0.165 & 0.097 & 747,900   & N/A & N/A & 0.706 & 0.841 & 0.772 & 1.255 \\
    \texttt{Dolly-v2-3B} & 0.828 & 0.58  & 0.493 & 0.29  & 2,484,000 & N/A & N/A & 0.677 & 0.804 & 0.737 & 1.298 \\
    \texttt{Pythia-2.8B} & 0.265 & 0.186 & 0.158 & 0.093 & 742,000   & N/A & N/A & 0.714 & 0.852 & 0.781 & 1.243 \\
    \texttt{Gemma-2B} & 0.76  & 0.532 & 0.453 & 0.266 & 1,520,000 & N/A & N/A & 0.605 & 0.729 & 0.661 & 1.398 \\
    \texttt{Llama-3.2-1B} & 1.22  & 0.854 & 0.457 & 0.319 & 8,500,000 & N/A & N/A & 0.76  & 0.995 & 0.83  & 1.145 \\
    \texttt{Phi-3} & 1.074 & 0.752 & 0.413 & 0.298 & 7,200,000 & N/A & N/A & 0.745 & 0.97  & 0.815 & 1.160 \\
    \texttt{Gemma-3} & 1.234 & 0.864 & 0.456 & 0.32  & 6,800,000 & N/A & N/A & 0.735 & 0.95  & 0.8   & 1.175 \\
    \bottomrule
    \end{tabularx}
    \caption{Detailed Results, \textbf{viggo}, \textbf{L4} GPU}
    \label{tab:app-models}
\end{table*}
